Development, Validation, and Benchmarking of a Multidisciplinary Semi-Analytical Model for Wave Energy Converters

Wave energy converters (WECs) require system-level techno-economic analysis to balance power production, cost, and survivability. Existing simulation tools are either too computationally costly for large-scale optimization or too narrow in disciplinary scope to support integrated design studies. This work presents MDOcean, a novel open-source WEC simulation framework for rapid early-stage design exploration, parametric analysis, and multidisciplinary optimization. MDOcean integrates hydrodynamics, dynamics, structures, and economics in a computationally efficient architecture based on analytical and semi-analytical methods that substantially reduce runtime while maintaining near-numerical accuracy. The framework includes an eigenfunction-based linear hydrodynamic solver, a quasi-linearized frequency-domain dynamics engine capable of modeling drag and saturation nonlinearities, a structural sizing module incorporating realistic yield, ultimate, buckling, storm, and fatigue design criteria, and a simple cost model for techno-economic assessment. Particular emphasis is placed on the linearized pseudo-spectral optimal control formulation, which extends frequency-domain constraint-handling approaches with a unified describing-function and analytical quadratically-constrained quadratic program framework. This formulation efficiently treats nonlinearities and constraints while preserving compatibility with optimization and frequency-domain analysis techniques. Validation and benchmarking demonstrate that MDOcean's 151 ms runtime is orders of magnitude faster than leading WEC simulation tools while maintaining agreement with higher-fidelity baselines to within a few percent in most cases. The framework also provides insight into limiting behaviors, scaling laws, subsystem interactions, and key tradeoffs governing WEC design and techno-economic performance.

==> numeric-results.tex <==
\makeatletter%
\newcommand\resultsAOR[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\resultsAOR@out{%
    \{%
      "forceScaleFactor": "0.28", %
      "powerScaleFactor": "0.49", %
      "massScaleFactor": "1.12", %
      "postpro\_time": 289.096547, %
      "analysis\_time": 2125.897354, %
      "nominalLCOE": "0.89 \$/kWh", %
      "surgeForceFloatNominal": "10 MN", %
      "surgeForceSparNominal": "3 MN", %
      "capexDesignNominal": 2190114.3223833465, %
      "powerAvgNominal": 72822.42633091437, %
      "simRuntime": "151 ms", %
      "pctRuntimeDynamics": "23\%", %
      "pctRuntimeMEEM": "70\%", %
      "pctRuntimeOther": "8\%", %
      "percent\_nans": 14.142661179698218, %
      "n\_geoms": 486, %
      "geom\_sweep\_analysis\_time": 199.131819, %
      "ptoSweepMinLCOE\_F\_max": "6.00 MN", %
      "ptoSweepMinLCOE\_P\_max": "400 kW", %
      "ptoSweepMinLCOE\_power": "76 kW", %
      "ptoSweepMinLCOE\_cost": "2.25 \$M", %
      "ptoSweepMinLCOE\_LCOE": "0.86 \$/kWh", %
      "err\_structs": {[}%
        \{%
          "pct\_error\_baseline": {[}%
            36.46449630326281, %
            38.53447655036626%
          {]}, %
          "pct\_error\_drag": {[}%
            10.790884267350611, %
            5.002294575560603%
          {]}, %
          "pct\_error\_meem": {[}%
            16.86150791429175, %
            66.75213581378641%
          {]}, %
          "pct\_error\_total": {[}%
            {-}12.715966046141702, %
            5.090339861457585%
          {]}%
        \}, %
        \{%
          "pct\_error\_baseline": {[}%
            {-}0.16459450665159717, %
            {-}0.06661021298838696%
          {]}, %
          "pct\_error\_drag": {[}%
            5.756780832854308, %
            {-}4.8276990600241785%
          {]}, %
          "pct\_error\_meem": {[}%
            {-}0.2782751787901601, %
            5.9001055035454675%
          {]}, %
          "pct\_error\_total": {[}%
            {-}2.0486004608632875, %
            {-}6.27926538734057%
          {]}%
        \}, %
        \{%
          "pct\_error\_baseline": {[}%
            36.49457444223329, %
            {-}27.657557186404567, %
            null, %
            null%
          {]}, %
          "pct\_error\_drag": {[}%
            65.47109436867538, %
            {-}11.439039626615637, %
            null, %
            null%
          {]}, %
          "pct\_error\_meem": {[}%
            36.49457444223329, %
            {-}32.7477682461545, %
            null, %
            null%
          {]}, %
          "pct\_error\_total": {[}%
            65.47109436867538, %
            {-}10.810656387995564, %
            null, %
            null%
          {]}%
        \}%
      {]}, %
      "wecsimAvgPowerErrorBestCase": "0.16\%", %
      "wecsimAvgPowerErrorWorstCase": "12.72\%", %
      "MEEMRuntime": "105 ms", %
      "meemSweepTime": "3 minutes", %
      "meemSweepSize": "6804"%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{forceScaleFactor}=0%
      \def\resultsAOR@out{%
    0.28}%
    \else%
      \ifnum\pdfstrcmp{#1}{powerScaleFactor}=0%
      \def\resultsAOR@out{%
    0.49}%
    \else%
      \ifnum\pdfstrcmp{#1}{massScaleFactor}=0%
      \def\resultsAOR@out{%
    1.12}%
    \else%
      \ifnum\pdfstrcmp{#1}{postpro_time}=0%
      \def\resultsAOR@out{%
    289.096547}%
    \else%
      \ifnum\pdfstrcmp{#1}{analysis_time}=0%
      \def\resultsAOR@out{%
    2125.897354}%
    \else%
      \ifnum\pdfstrcmp{#1}{nominalLCOE}=0%
      \def\resultsAOR@out{%
    0.89 \$/kWh}%
    \else%
      \ifnum\pdfstrcmp{#1}{surgeForceFloatNominal}=0%
      \def\resultsAOR@out{%
    10 MN}%
    \else%
      \ifnum\pdfstrcmp{#1}{surgeForceSparNominal}=0%
      \def\resultsAOR@out{%
    3 MN}%
    \else%
      \ifnum\pdfstrcmp{#1}{capexDesignNominal}=0%
      \def\resultsAOR@out{%
    2190114.3223833465}%
    \else%
      \ifnum\pdfstrcmp{#1}{powerAvgNominal}=0%
      \def\resultsAOR@out{%
    72822.42633091437}%
    \else%
      \ifnum\pdfstrcmp{#1}{simRuntime}=0%
      \def\resultsAOR@out{%
    151 ms}%
    \else%
      \ifnum\pdfstrcmp{#1}{pctRuntimeDynamics}=0%
      \def\resultsAOR@out{%
    23\%}%
    \else%
      \ifnum\pdfstrcmp{#1}{pctRuntimeMEEM}=0%
      \def\resultsAOR@out{%
    70\%}%
    \else%
      \ifnum\pdfstrcmp{#1}{pctRuntimeOther}=0%
      \def\resultsAOR@out{%
    8\%}%
    \else%
      \ifnum\pdfstrcmp{#1}{percent_nans}=0%
      \def\resultsAOR@out{%
    14.142661179698218}%
    \else%
      \ifnum\pdfstrcmp{#1}{n_geoms}=0%
      \def\resultsAOR@out{%
    486}%
    \else%
      \ifnum\pdfstrcmp{#1}{geom_sweep_analysis_time}=0%
      \def\resultsAOR@out{%
    199.131819}%
    \else%
      \ifnum\pdfstrcmp{#1}{ptoSweepMinLCOE_F_max}=0%
      \def\resultsAOR@out{%
    6.00 MN}%
    \else%
      \ifnum\pdfstrcmp{#1}{ptoSweepMinLCOE_P_max}=0%
      \def\resultsAOR@out{%
    400 kW}%
    \else%
      \ifnum\pdfstrcmp{#1}{ptoSweepMinLCOE_power}=0%
      \def\resultsAOR@out{%
    76 kW}%
    \else%
      \ifnum\pdfstrcmp{#1}{ptoSweepMinLCOE_cost}=0%
      \def\resultsAOR@out{%
    2.25 \$M}%
    \else%
      \ifnum\pdfstrcmp{#1}{ptoSweepMinLCOE_LCOE}=0%
      \def\resultsAOR@out{%
    0.86 \$/kWh}%
    \else%
      \ifnum\pdfstrcmp{#1}{err_structs}=0%
      \let\resultsAOR@out\resultsAOR@I%
    \else%
      \ifnum\pdfstrcmp{#1}{wecsimAvgPowerErrorBestCase}=0%
      \def\resultsAOR@out{%
    0.16\%}%
    \else%
      \ifnum\pdfstrcmp{#1}{wecsimAvgPowerErrorWorstCase}=0%
      \def\resultsAOR@out{%
    12.72\%}%
    \else%
      \ifnum\pdfstrcmp{#1}{MEEMRuntime}=0%
      \def\resultsAOR@out{%
    105 ms}%
    \else%
      \ifnum\pdfstrcmp{#1}{meemSweepTime}=0%
      \def\resultsAOR@out{%
    3 minutes}%
    \else%
      \ifnum\pdfstrcmp{#1}{meemSweepSize}=0%
      \def\resultsAOR@out{%
    6804}%
    \else%
      \def\resultsAOR@out{%
    ??}%
    \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
  \fi
  \resultsAOR@out
}\newcommand\resultsAOR@I[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\resultsAOR@I@out{%
    {[}%
      \{%
        "pct\_error\_baseline": {[}%
          36.46449630326281, %
          38.53447655036626%
        {]}, %
        "pct\_error\_drag": {[}%
          10.790884267350611, %
          5.002294575560603%
        {]}, %
        "pct\_error\_meem": {[}%
          16.86150791429175, %
          66.75213581378641%
        {]}, %
        "pct\_error\_total": {[}%
          {-}12.715966046141702, %
          5.090339861457585%
        {]}%
      \}, %
      \{%
        "pct\_error\_baseline": {[}%
          {-}0.16459450665159717, %
          {-}0.06661021298838696%
        {]}, %
        "pct\_error\_drag": {[}%
          5.756780832854308, %
          {-}4.8276990600241785%
        {]}, %
        "pct\_error\_meem": {[}%
          {-}0.2782751787901601, %
          5.9001055035454675%
        {]}, %
        "pct\_error\_total": {[}%
          {-}2.0486004608632875, %
          {-}6.27926538734057%
        {]}%
      \}, %
      \{%
        "pct\_error\_baseline": {[}%
          36.49457444223329, %
          {-}27.657557186404567, %
          null, %
          null%
        {]}, %
        "pct\_error\_drag": {[}%
          65.47109436867538, %
          {-}11.439039626615637, %
          null, %
          null%
        {]}, %
        "pct\_error\_meem": {[}%
          36.49457444223329, %
          {-}32.7477682461545, %
          null, %
          null%
        {]}, %
        "pct\_error\_total": {[}%
          65.47109436867538, %
          {-}10.810656387995564, %
          null, %
          null%
        {]}%
      \}%
    {]}}%
  \else%
    \ifnum\pdfstrcmp{#1}{0}=0%
      \let\resultsAOR@I@out\resultsAOR@II%
    \else%
      \ifnum\pdfstrcmp{#1}{1}=0%
      \let\resultsAOR@I@out\resultsAOR@III%
    \else%
      \ifnum\pdfstrcmp{#1}{2}=0%
      \let\resultsAOR@I@out\resultsAOR@IV%
    \else%
      \def\resultsAOR@I@out{%
    ??}%
    \fi\fi\fi
  \fi
  \resultsAOR@I@out
}\newcommand\resultsAOR@II[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\resultsAOR@II@out{%
    \{%
      "pct\_error\_baseline": {[}%
        36.46449630326281, %
        38.53447655036626%
      {]}, %
      "pct\_error\_drag": {[}%
        10.790884267350611, %
        5.002294575560603%
      {]}, %
      "pct\_error\_meem": {[}%
        16.86150791429175, %
        66.75213581378641%
      {]}, %
      "pct\_error\_total": {[}%
        {-}12.715966046141702, %
        5.090339861457585%
      {]}%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{pct_error_baseline}=0%
      \let\resultsAOR@II@out\resultsAOR@V%
    \else%
      \ifnum\pdfstrcmp{#1}{pct_error_drag}=0%
      \let\resultsAOR@II@out\resultsAOR@VI%
    \else%
      \ifnum\pdfstrcmp{#1}{pct_error_meem}=0%
      \let\resultsAOR@II@out\resultsAOR@VII%
    \else%
      \ifnum\pdfstrcmp{#1}{pct_error_total}=0%
      \let\resultsAOR@II@out\resultsAOR@VIII%
    \else%
      \def\resultsAOR@II@out{%
    ??}%
    \fi\fi\fi\fi
  \fi
  \resultsAOR@II@out
}\newcommand\resultsAOR@III[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\resultsAOR@III@out{%
    \{%
      "pct\_error\_baseline": {[}%
        {-}0.16459450665159717, %
        {-}0.06661021298838696%
      {]}, %
      "pct\_error\_drag": {[}%
        5.756780832854308, %
        {-}4.8276990600241785%
      {]}, %
      "pct\_error\_meem": {[}%
        {-}0.2782751787901601, %
        5.9001055035454675%
      {]}, %
      "pct\_error\_total": {[}%
        {-}2.0486004608632875, %
        {-}6.27926538734057%
      {]}%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{pct_error_baseline}=0%
      \let\resultsAOR@III@out\resultsAOR@IX%
    \else%
      \ifnum\pdfstrcmp{#1}{pct_error_drag}=0%
      \let\resultsAOR@III@out\resultsAOR@X%
    \else%
      \ifnum\pdfstrcmp{#1}{pct_error_meem}=0%
      \let\resultsAOR@III@out\resultsAOR@XI%
    \else%
      \ifnum\pdfstrcmp{#1}{pct_error_total}=0%
      \let\resultsAOR@III@out\resultsAOR@XII%
    \else%
      \def\resultsAOR@III@out{%
    ??}%
    \fi\fi\fi\fi
  \fi
  \resultsAOR@III@out
}\newcommand\resultsAOR@IV[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\resultsAOR@IV@out{%
    \{%
      "pct\_error\_baseline": {[}%
        36.49457444223329, %
        {-}27.657557186404567, %
        null, %
        null%
      {]}, %
      "pct\_error\_drag": {[}%
        65.47109436867538, %
        {-}11.439039626615637, %
        null, %
        null%
      {]}, %
      "pct\_error\_meem": {[}%
        36.49457444223329, %
        {-}32.7477682461545, %
        null, %
        null%
      {]}, %
      "pct\_error\_total": {[}%
        65.47109436867538, %
        {-}10.810656387995564, %
        null, %
        null%
      {]}%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{pct_error_baseline}=0%
      \let\resultsAOR@IV@out\resultsAOR@XIII%
    \else%
      \ifnum\pdfstrcmp{#1}{pct_error_drag}=0%
      \let\resultsAOR@IV@out\resultsAOR@XIV%
    \else%
      \ifnum\pdfstrcmp{#1}{pct_error_meem}=0%
      \let\resultsAOR@IV@out\resultsAOR@XV%
    \else%
      \ifnum\pdfstrcmp{#1}{pct_error_total}=0%
      \let\resultsAOR@IV@out\resultsAOR@XVI%
    \else%
      \def\resultsAOR@IV@out{%
    ??}%
    \fi\fi\fi\fi
  \fi
  \resultsAOR@IV@out
}\newcommand\resultsAOR@V[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\resultsAOR@V@out{%
    {[}%
      36.46449630326281, %
      38.53447655036626%
    {]}}%
  \else%
    \ifnum\pdfstrcmp{#1}{0}=0%
      \def\resultsAOR@V@out{%
    36.46449630326281}%
    \else%
      \ifnum\pdfstrcmp{#1}{1}=0%
      \def\resultsAOR@V@out{%
    38.53447655036626}%
    \else%
      \def\resultsAOR@V@out{%
    ??}%
    \fi\fi
  \fi
  \resultsAOR@V@out
}\newcommand\resultsAOR@VI[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\resultsAOR@VI@out{%
    {[}%
      10.790884267350611, %
      5.002294575560603%
    {]}}%
  \else%
    \ifnum\pdfstrcmp{#1}{0}=0%
      \def\resultsAOR@VI@out{%
    10.790884267350611}%
    \else%
      \ifnum\pdfstrcmp{#1}{1}=0%
      \def\resultsAOR@VI@out{%
    5.002294575560603}%
    \else%
      \def\resultsAOR@VI@out{%
    ??}%
    \fi\fi
  \fi
  \resultsAOR@VI@out
}\newcommand\resultsAOR@VII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\resultsAOR@VII@out{%
    {[}%
      16.86150791429175, %
      66.75213581378641%
    {]}}%
  \else%
    \ifnum\pdfstrcmp{#1}{0}=0%
      \def\resultsAOR@VII@out{%
    16.86150791429175}%
    \else%
      \ifnum\pdfstrcmp{#1}{1}=0%
      \def\resultsAOR@VII@out{%
    66.75213581378641}%
    \else%
      \def\resultsAOR@VII@out{%
    ??}%
    \fi\fi
  \fi
  \resultsAOR@VII@out
}\newcommand\resultsAOR@VIII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\resultsAOR@VIII@out{%
    {[}%
      {-}12.715966046141702, %
      5.090339861457585%
    {]}}%
  \else%
    \ifnum\pdfstrcmp{#1}{0}=0%
      \def\resultsAOR@VIII@out{%
    {-}12.715966046141702}%
    \else%
      \ifnum\pdfstrcmp{#1}{1}=0%
      \def\resultsAOR@VIII@out{%
    5.090339861457585}%
    \else%
      \def\resultsAOR@VIII@out{%
    ??}%
    \fi\fi
  \fi
  \resultsAOR@VIII@out
}\newcommand\resultsAOR@IX[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\resultsAOR@IX@out{%
    {[}%
      {-}0.16459450665159717, %
      {-}0.06661021298838696%
    {]}}%
  \else%
    \ifnum\pdfstrcmp{#1}{0}=0%
      \def\resultsAOR@IX@out{%
    {-}0.16459450665159717}%
    \else%
      \ifnum\pdfstrcmp{#1}{1}=0%
      \def\resultsAOR@IX@out{%
    {-}0.06661021298838696}%
    \else%
      \def\resultsAOR@IX@out{%
    ??}%
    \fi\fi
  \fi
  \resultsAOR@IX@out
}\newcommand\resultsAOR@X[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\resultsAOR@X@out{%
    {[}%
      5.756780832854308, %
      {-}4.8276990600241785%
    {]}}%
  \else%
    \ifnum\pdfstrcmp{#1}{0}=0%
      \def\resultsAOR@X@out{%
    5.756780832854308}%
    \else%
      \ifnum\pdfstrcmp{#1}{1}=0%
      \def\resultsAOR@X@out{%
    {-}4.8276990600241785}%
    \else%
      \def\resultsAOR@X@out{%
    ??}%
    \fi\fi
  \fi
  \resultsAOR@X@out
}\newcommand\resultsAOR@XI[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\resultsAOR@XI@out{%
    {[}%
      {-}0.2782751787901601, %
      5.9001055035454675%
    {]}}%
  \else%
    \ifnum\pdfstrcmp{#1}{0}=0%
      \def\resultsAOR@XI@out{%
    {-}0.2782751787901601}%
    \else%
      \ifnum\pdfstrcmp{#1}{1}=0%
      \def\resultsAOR@XI@out{%
    5.9001055035454675}%
    \else%
      \def\resultsAOR@XI@out{%
    ??}%
    \fi\fi
  \fi
  \resultsAOR@XI@out
}\newcommand\resultsAOR@XII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\resultsAOR@XII@out{%
    {[}%
      {-}2.0486004608632875, %
      {-}6.27926538734057%
    {]}}%
  \else%
    \ifnum\pdfstrcmp{#1}{0}=0%
      \def\resultsAOR@XII@out{%
    {-}2.0486004608632875}%
    \else%
      \ifnum\pdfstrcmp{#1}{1}=0%
      \def\resultsAOR@XII@out{%
    {-}6.27926538734057}%
    \else%
      \def\resultsAOR@XII@out{%
    ??}%
    \fi\fi
  \fi
  \resultsAOR@XII@out
}\newcommand\resultsAOR@XIII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\resultsAOR@XIII@out{%
    {[}%
      36.49457444223329, %
      {-}27.657557186404567, %
      null, %
      null%
    {]}}%
  \else%
    \ifnum\pdfstrcmp{#1}{0}=0%
      \def\resultsAOR@XIII@out{%
    36.49457444223329}%
    \else%
      \ifnum\pdfstrcmp{#1}{1}=0%
      \def\resultsAOR@XIII@out{%
    {-}27.657557186404567}%
    \else%
      \ifnum\pdfstrcmp{#1}{2}=0%
      \def\resultsAOR@XIII@out{%
    None}%
    \else%
      \ifnum\pdfstrcmp{#1}{3}=0%
      \def\resultsAOR@XIII@out{%
    None}%
    \else%
      \def\resultsAOR@XIII@out{%
    ??}%
    \fi\fi\fi\fi
  \fi
  \resultsAOR@XIII@out
}\newcommand\resultsAOR@XIV[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\resultsAOR@XIV@out{%
    {[}%
      65.47109436867538, %
      {-}11.439039626615637, %
      null, %
      null%
    {]}}%
  \else%
    \ifnum\pdfstrcmp{#1}{0}=0%
      \def\resultsAOR@XIV@out{%
    65.47109436867538}%
    \else%
      \ifnum\pdfstrcmp{#1}{1}=0%
      \def\resultsAOR@XIV@out{%
    {-}11.439039626615637}%
    \else%
      \ifnum\pdfstrcmp{#1}{2}=0%
      \def\resultsAOR@XIV@out{%
    None}%
    \else%
      \ifnum\pdfstrcmp{#1}{3}=0%
      \def\resultsAOR@XIV@out{%
    None}%
    \else%
      \def\resultsAOR@XIV@out{%
    ??}%
    \fi\fi\fi\fi
  \fi
  \resultsAOR@XIV@out
}\newcommand\resultsAOR@XV[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\resultsAOR@XV@out{%
    {[}%
      36.49457444223329, %
      {-}32.7477682461545, %
      null, %
      null%
    {]}}%
  \else%
    \ifnum\pdfstrcmp{#1}{0}=0%
      \def\resultsAOR@XV@out{%
    36.49457444223329}%
    \else%
      \ifnum\pdfstrcmp{#1}{1}=0%
      \def\resultsAOR@XV@out{%
    {-}32.7477682461545}%
    \else%
      \ifnum\pdfstrcmp{#1}{2}=0%
      \def\resultsAOR@XV@out{%
    None}%
    \else%
      \ifnum\pdfstrcmp{#1}{3}=0%
      \def\resultsAOR@XV@out{%
    None}%
    \else%
      \def\resultsAOR@XV@out{%
    ??}%
    \fi\fi\fi\fi
  \fi
  \resultsAOR@XV@out
}\newcommand\resultsAOR@XVI[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\resultsAOR@XVI@out{%
    {[}%
      65.47109436867538, %
      {-}10.810656387995564, %
      null, %
      null%
    {]}}%
  \else%
    \ifnum\pdfstrcmp{#1}{0}=0%
      \def\resultsAOR@XVI@out{%
    65.47109436867538}%
    \else%
      \ifnum\pdfstrcmp{#1}{1}=0%
      \def\resultsAOR@XVI@out{%
    {-}10.810656387995564}%
    \else%
      \ifnum\pdfstrcmp{#1}{2}=0%
      \def\resultsAOR@XVI@out{%
    None}%
    \else%
      \ifnum\pdfstrcmp{#1}{3}=0%
      \def\resultsAOR@XVI@out{%
    None}%
    \else%
      \def\resultsAOR@XVI@out{%
    ??}%
    \fi\fi\fi\fi
  \fi
  \resultsAOR@XVI@out
}%
\makeatother%
